dMVX: Secure and Efficient Multi-Variant Execution in a Distributed Setting

Multi-variant execution (MVX) systems amplify the effectiveness of software diversity techniques. The key idea is to run multiple diversified program variants in lockstep while providing them with the same input and monitoring their run-time behavior for divergences. Thus, adversaries have to compromise all program variants simultaneously to mount an attack successfully. Recent work proposed distributed, heterogeneous MVX systems that leverage different ABIs and ISAs to increase the diversity between program variants further. However, existing distributed MVX system designs suffer from high performance overhead due to time-consuming network transactions for the MVX system's operations. This paper presents dMVX, a novel hybrid distributed MVX design, which incorporates new techniques that significantly reduce the overhead of MVX systems in a distributed setting. Our key insight is that we can intelligently reduce the MVX operations that use expensive network transfers. First, we can limit the monitoring of system calls that are not security-critical. Second, we observe that, in many circumstances, we can also safely cache or avoid replication operations needed for I/O related system calls. Our evaluation shows that dMVX reduces the performance degradation from over 50% to 3.1% for realistic server benchmarks.

==> relatedwork.tex <==
\section{Related Work}

Here I need to make clear the differences with DMON + the virginia people work
+ remon and also stretch the fact that this is the first monitor that needs to do system calls
for monitoring and replication.


